Comments on the little string partition functions of $K3\times T^2$ via the refined topological vertex

We compute partition functions of the deformed multiple M5-branes theory on $K3\times T^2$ using the refined topological vertex formalism and the Borcherds lift. The deformation is related to the mass deformation in the corresponding four dimensional $N=4$ $SU(N)$ gauge theory on $K3$. The seed of the Borcherd-lift is calculated by taking the universal part of the type IIb little string free energy of the CY3-fold $X_{N,1}$. We provide explicit modular covariant expressions, as expansions in the mass parameter $m$, of the genus two Siegel modular forms produced by the Borcherds lift of the first few seed functions. We also discuss the relation between genus-one free energy and Ray-Singer Torsion, and the automorphic properties of the latter.

==> bibliography.tex <==

@article{Hohenegger:2013ala,
    author = "Hohenegger, Stefan and Iqbal, Amer",
    title = "{M-strings, elliptic genera and $\mathcal{N} = 4$ string amplitudes}",
    eprint = "1310.1325",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "CERN-PH-TH-2013-237",
    doi = "10.1002/prop.201300035",
    journal = "Fortsch. Phys.",
    volume = "62",
    pages = "155--206",
    year = "2014"
}
@inproceedings{Gritsenko:1999nm,
    author = "Gritsenko, V.",
    title = "{Complex vector bundles and Jacobi forms}",
    eprint = "math/9906191",
    archivePrefix = "arXiv",
    month = "1",
    year = "1999"
}
@ARTICLE{1998math......6011G,
       author = {{Gritsenko}, V. and {Hulek}, K.},
        title = "{The Modular Form of the Barth-Nieto Quintic}",
      journal = {arXiv Mathematics e-prints},
     keywords = {Algebraic Geometry},
         year = 1998,
        month = jun,
          eid = {math/9806011},
        pages = {math/9806011},
archivePrefix = {arXiv},
       eprint = {math/9806011},
 primaryClass = {math.AG},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998math......6011G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Harvey:1996ts,
    author = "Harvey, Jeffrey A. and Moore, Gregory W.",
    title = "{Exact gravitational threshold correction in the FHSV model}",
    eprint = "hep-th/9611176",
    archivePrefix = "arXiv",
    reportNumber = "EFI-96-40, YCTP-P22-96",
    doi = "10.1103/PhysRevD.57.2329",
    journal = "Phys. Rev. D",
    volume = "57",
    pages = "2329--2336",
    year = "1998"
}
@article{Govindarajan:2010fu,
    author = "Govindarajan, Suresh",
    title = "{BKM Lie superalgebras from counting twisted CHL dyons}",
    eprint = "1006.3472",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "IITM-PH-TH-2010-5",
    doi = "10.1007/JHEP05(2011)089",
    journal = "JHEP",
    volume = "05",
    pages = "089",
    year = "2011"
}
@article{Dijkgraaf:2002yn,
    author = "Dijkgraaf, Robbert and Sinkovics, Annamaria and Temurhan, Mine",
    title = "{Matrix models and gravitational corrections}",
    eprint = "hep-th/0211241",
    archivePrefix = "arXiv",
    reportNumber = "ITFA-2002-53",
    doi = "10.4310/ATMP.2003.v7.n6.a7",
    journal = "Adv. Theor. Math. Phys.",
    volume = "7",
    number = "6",
    pages = "1155--1174",
    year = "2003"
}
@article{Iqbal:2003ds,
    author = "Iqbal, Amer and Nekrasov, Nikita and Okounkov, Andrei and Vafa, Cumrun",
    title = "{Quantum foam and topological strings}",
    eprint = "hep-th/0312022",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-03-A078, IHES-P-03-65, ITEP-TH-60-03",
    doi = "10.1088/1126-6708/2008/04/011",
    journal = "JHEP",
    volume = "04",
    pages = "011",
    year = "2008"
}
@article{Hohenegger:2016eqy,
    author = "Hohenegger, Stefan and Iqbal, Amer and Rey, Soo-Jong",
    title = "{Self-Duality and Self-Similarity of Little String Orbifolds}",
    eprint = "1605.02591",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.94.046006",
    journal = "Phys. Rev. D",
    volume = "94",
    number = "4",
    pages = "046006",
    year = "2016"
}

@article{Hohenegger:2015btj,
    author = "Hohenegger, Stefan and Iqbal, Amer and Rey, Soo-Jong",
    title = "{Instanton-monopole correspondence from M-branes on $\mathbb S^1$ and little string theory}",
    eprint = "1511.02787",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.93.066016",
    journal = "Phys. Rev. D",
    volume = "93",
    number = "6",
    pages = "066016",
    year = "2016"
}
@article{Dijkgraaf:2007sw,
    author = "Dijkgraaf, Robbert and Hollands, Lotte and Sulkowski, Piotr and Vafa, Cumrun",
    title = "{Supersymmetric gauge theories, intersecting branes and free fermions}",
    eprint = "0709.4446",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "HUTP-07-A006, ITFA-2007-44, IFT-UW-2007-9",
    doi = "10.1088/1126-6708/2008/02/106",
    journal = "JHEP",
    volume = "02",
    pages = "106",
    year = "2008"
}

@article{Harvey:2014nha,
    author = "Harvey, Jeffrey A. and Lee, Sungjay and Murthy, Sameer",
    title = "{Elliptic genera of ALE and ALF manifolds from gauged linear sigma models}",
    eprint = "1406.6342",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "EFI-14-10",
    doi = "10.1007/JHEP02(2015)110",
    journal = "JHEP",
    volume = "02",
    pages = "110",
    year = "2015"
}

@article{Dijkgraaf:2002ac,
    author = "Dijkgraaf, Robbert and Verlinde, Erik P. and Vonk, Marcel",
    title = "{On the partition sum of the NS five-brane}",
    eprint = "hep-th/0205281",
    archivePrefix = "arXiv",
    reportNumber = "PUPT-2030, SPIN-2002-10, ITFA-2002-9",
    month = "5",
    year = "2002"
}
@article{Dijkgraaf:1996it,
    author = "Dijkgraaf, Robbert and Verlinde, Erik P. and Verlinde, Herman L.",
    title = "{Counting dyons in N=4 string theory}",
    eprint = "hep-th/9607026",
    archivePrefix = "arXiv",
    reportNumber = "CERN-TH-96-170",
    doi = "10.1016/S0550-3213(96)00640-2",
    journal = "Nucl. Phys. B",
    volume = "484",
    pages = "543--561",
    year = "1997"
}

@article{Dijkgraaf:1996xw,
    author = "Dijkgraaf, Robbert and Moore, Gregory W. and Verlinde, Erik P. and Verlinde, Herman L.",
    title = "{Elliptic genera of symmetric products and second quantized strings}",
    eprint = "hep-th/9608096",
    archivePrefix = "arXiv",
    reportNumber = "CERN-TH-96-222, ITFA-96-31, YCTP-P16-96",
    doi = "10.1007/s002200050087",
    journal = "Commun. Math. Phys.",
    volume = "185",
    pages = "197--209",
    year = "1997"
}
@ARTICLE{1999math......4092Y,
       author = {{Yoshikawa}, Ken-Ichi},
        title = "{Discriminant of theta divisors and Quillen metrics}",
      journal = {arXiv Mathematics e-prints},
     keywords = {Algebraic Geometry},
         year = 1999,
        month = apr,
          eid = {math/9904092},
        pages = {math/9904092},
archivePrefix = {arXiv},
       eprint = {math/9904092},
 primaryClass = {math.AG},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999math......4092Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Hohenegger:2015cba,
    author = "Hohenegger, Stefan and Iqbal, Amer and Rey, Soo-Jong",
    title = "{M-strings, monopole strings, and modular forms}",
    eprint = "1503.06983",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "SNUST-15-02",
    doi = "10.1103/PhysRevD.92.066005",
    journal = "Phys. Rev. D",
    volume = "92",
    number = "6",
    pages = "066005",
    year = "2015"
}

@article{Iqbal:2007ii,
    author = "Iqbal, Amer and Kozcaz, Can and Vafa, Cumrun",
    title = "{The Refined topological vertex}",
    eprint = "hep-th/0701156",
    archivePrefix = "arXiv",
    doi = "10.1088/1126-6708/2009/10/069",
    journal = "JHEP",
    volume = "10",
    pages = "069",
    year = "2009"
}
@article{Aoki2005SIMPLEGR,
  title={SIMPLE GRADED RINGS OF SIEGEL MODULAR FORMS, DIFFERENTIAL OPERATORS AND BORCHERDS PRODUCTS},
  author={Hiroki Aoki and T. Ibukiyama},
  journal={International Journal of Mathematics},
  year={2005},
  volume={16},
  pages={249-279}
}
@article{Dabholkar:2006xa,
    author = "Dabholkar, Atish and Nampuri, Suresh",
    title = "{Spectrum of dyons and black holes in CHL orbifolds using Borcherds lift}",
    eprint = "hep-th/0603066",
    archivePrefix = "arXiv",
    reportNumber = "TIFR-TH-06-07",
    doi = "10.1088/1126-6708/2007/11/077",
    journal = "JHEP",
    volume = "11",
    pages = "077",
    year = "2007"
}
@article{Vafa:1994tf,
    author = "Vafa, Cumrun and Witten, Edward",
    title = "{A Strong coupling test of S duality}",
    eprint = "hep-th/9408074",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-94-A017, IASSNS-HEP-94-54",
    doi = "10.1016/0550-3213(94)90097-3",
    journal = "Nucl. Phys. B",
    volume = "431",
    pages = "3--77",
    year = "1994"
}
@article{Marcus:1995mq,
    author = "Marcus, Neil",
    title = "{The Other topological twisting of N=4 Yang-Mills}",
    eprint = "hep-th/9506002",
    archivePrefix = "arXiv",
    reportNumber = "TAUP-2247-95",
    doi = "10.1016/0550-3213(95)00389-A",
    journal = "Nucl. Phys. B",
    volume = "452",
    pages = "331--345",
    year = "1995"
}

@article{Cordes:1994sd,
    author = "Cordes, Stefan and Moore, Gregory W. and Ramgoolam, Sanjaye",
    title = "{Large N 2-D Yang-Mills theory and topological string theory}",
    eprint = "hep-th/9402107",
    archivePrefix = "arXiv",
    reportNumber = "YCTP-P23-93, RU-94-20",
    doi = "10.1007/s002200050102",
    journal = "Commun. Math. Phys.",
    volume = "185",
    pages = "543--619",
    year = "1997"
}

@article{Labastida:1997xk,
    author = "Labastida, J. M. F. and Lozano, Carlos",
    title = "{Mass perturbations in twisted N=4 supersymmetric gauge theories}",
    eprint = "hep-th/9711132",
    archivePrefix = "arXiv",
    reportNumber = "CERN-TH-97-316, US-FT-33-97",
    doi = "10.1016/S0550-3213(98)00135-7",
    journal = "Nucl. Phys. B",
    volume = "518",
    pages = "37--58",
    year = "1998"
}
@article{Labastida:1997vq,
    author = "Labastida, J. M. F. and Lozano, Carlos",
    title = "{Mathai-Quillen formulation of twisted N=4 supersymmetric gauge theories in four-dimensions}",
    eprint = "hep-th/9702106",
    archivePrefix = "arXiv",
    reportNumber = "US-FT-4-97",
    doi = "10.1016/S0550-3213(97)00421-5",
    journal = "Nucl. Phys. B",
    volume = "502",
    pages = "741--790",
    year = "1997"
}

@phdthesis{Marino:1996sd,
    author = "Marino, Marcos",
    title = "{The Geometry of supersymmetric gauge theories in four-dimensions}",
    eprint = "hep-th/9701128",
    archivePrefix = "arXiv",
    reportNumber = "US-FT-2-97",
    school = "Santiago de Compostela U.",
    year = "1997"
}
@article{Haghighat:2013gba,
    author = "Haghighat, Babak and Iqbal, Amer and Koz\c{c}az, Can and Lockhart, Guglielmo and Vafa, Cumrun",
    title = "{M-Strings}",
    eprint = "1305.6322",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/s00220-014-2139-1",
    journal = "Commun. Math. Phys.",
    volume = "334",
    number = "2",
    pages = "779--842",
    year = "2015"
}
@article{Haghighat:2013tka,
    author = "Haghighat, Babak and Kozcaz, Can and Lockhart, Guglielmo and Vafa, Cumrun",
    title = "{Orbifolds of M-strings}",
    eprint = "1310.1185",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.89.046003",
    journal = "Phys. Rev. D",
    volume = "89",
    number = "4",
    pages = "046003",
    year = "2014"
}
@article{Hohenegger:2013ala,
    author = "Hohenegger, Stefan and Iqbal, Amer",
    title = "{M-strings, elliptic genera and $\mathcal{N} = 4$ string amplitudes}",
    eprint = "1310.1325",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "CERN-PH-TH-2013-237",
    doi = "10.1002/prop.201300035",
    journal = "Fortsch. Phys.",
    volume = "62",
    pages = "155--206",
    year = "2014"
}
@article{Kawai:2000px,
    author = "Kawai, Toshiya and Yoshioka, Kota",
    title = "{String partition functions and infinite products}",
    eprint = "hep-th/0002169",
    archivePrefix = "arXiv",
    doi = "10.4310/ATMP.2000.v4.n2.a7",
    journal = "Adv. Theor. Math. Phys.",
    volume = "4",
    pages = "397--485",
    year = "2000"
}
@article{Hollowood:2003cv,
    author = "Hollowood, Timothy J. and Iqbal, Amer and Vafa, Cumrun",
    title = "{Matrix models, geometric engineering and elliptic genera}",
    eprint = "hep-th/0310272",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-03-A074",
    doi = "10.1088/1126-6708/2008/03/069",
    journal = "JHEP",
    volume = "03",
    pages = "069",
    year = "2008"
}
@article{Nekrasov:2002qd,
    author = "Nekrasov, Nikita A.",
    title = "{Seiberg-Witten prepotential from instanton counting}",
    eprint = "hep-th/0206161",
    archivePrefix = "arXiv",
    reportNumber = "ITEP-TH-22-02, IHES-P-04-22",
    doi = "10.4310/ATMP.2003.v7.n5.a4",
    journal = "Adv. Theor. Math. Phys.",
    volume = "7",
    number = "5",
    pages = "831--864",
    year = "2003"
}
@inproceedings{Gritsenko:1999nm,
    author = "Gritsenko, V.",
    title = "{Complex vector bundles and Jacobi forms}",
    eprint = "math/9906191",
    archivePrefix = "arXiv",
    month = "1",
    year = "1999"
}
@article{Bershadsky:1993cx,
    author = "Bershadsky, M. and Cecotti, S. and Ooguri, H. and Vafa, C.",
    title = "{Kodaira-Spencer theory of gravity and exact results for quantum string amplitudes}",
    eprint = "hep-th/9309140",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-93-A025, RIMS-946, SISSA-142-93-EP",
    doi = "10.1007/BF02099774",
    journal = "Commun. Math. Phys.",
    volume = "165",
    pages = "311--428",
    year = "1994"
}
@article{Bershadsky:1993ta,
    author = "Bershadsky, M. and Cecotti, S. and Ooguri, H. and Vafa, C.",
    editor = "Greene, B. and Yau, Shing-Tung",
    title = "{Holomorphic anomalies in topological field theories}",
    eprint = "hep-th/9302103",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-93-A008, RIMS-915",
    doi = "10.1016/0550-3213(93)90548-4",
    journal = "Nucl. Phys. B",
    volume = "405",
    pages = "279--304",
    year = "1993"
}
@ARTICLE{2019arXiv190701535B,
       author = {{Bryan}, Jim and {Gyenge}, {\'A}d{\'a}m},
        title = "{$G$-fixed Hilbert schemes on $K3$ surfaces, modular forms, and eta products}",
      journal = {arXiv e-prints},
     keywords = {Mathematics - Algebraic Geometry, 14J28, 14C05, 11F03, 11F20, 11F27},
         year = 2019,
        month = jul,
          eid = {arXiv:1907.01535},
        pages = {arXiv:1907.01535},
archivePrefix = {arXiv},
       eprint = {1907.01535},
 primaryClass = {math.AG},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190701535B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{David:2006ji,
    author = "David, Justin R. and Jatkar, Dileep P. and Sen, Ashoke",
    title = "{Product representation of Dyon partition function in CHL models}",
    eprint = "hep-th/0602254",
    archivePrefix = "arXiv",
    doi = "10.1088/1126-6708/2006/06/064",
    journal = "JHEP",
    volume = "06",
    pages = "064",
    year = "2006"
}
@article{Aharony:1999ks,
    author = "Aharony, Ofer",
    editor = "Lechtenfeld, O. and Louis, J. and Lust, Dieter and Nicolai, H.",
    title = "{A Brief review of 'little string theories'}",
    eprint = "hep-th/9911147",
    archivePrefix = "arXiv",
    reportNumber = "RUNHETC-99-42",
    doi = "10.1088/0264-9381/17/5/302",
    journal = "Class. Quant. Grav.",
    volume = "17",
    pages = "929--938",
    year = "2000"
}
@article{Cecotti:1992vy,
    author = "Cecotti, Sergio and Vafa, Cumrun",
    title = "{Ising model and N=2 supersymmetric theories}",
    eprint = "hep-th/9209085",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-92-A044, SISSA-167-92-EP",
    doi = "10.1007/BF02098023",
    journal = "Commun. Math. Phys.",
    volume = "157",
    pages = "139--178",
    year = "1993"
}
@article{Gritsenko:1996tm,
    author = "Gritsenko, Valeri A. and Nikulin, Vyacheslav V.",
    title = "{Automorphic forms and Lorentzian Kac-Moody algebras. Part 2}",
    eprint = "alg-geom/9611028",
    archivePrefix = "arXiv",
    reportNumber = "RIMS-1122",
    month = "12",
    year = "1996"
}
@article{Dabholkar:2012nd,
    author = "Dabholkar, Atish and Murthy, Sameer and Zagier, Don",
    title = "{Quantum Black Holes, Wall Crossing, and Mock Modular Forms}",
    eprint = "1208.4074",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "8",
    year = "2012"
}
@book{eichler2013theory,
  title={The Theory of Jacobi Forms},
  author={Eichler, M. and Zagier, D.},
  isbn={9781468491623},
  lccn={84028250},
  series={Progress in Mathematics},
  url={https://books.google.com.pk/books?id=p\_PTBwAAQBAJ},
  year={2013},
  publisher={Birkh{\"a}user Boston}
}
@article{Belin:2019jqz,
    author = {Belin, Alexandre and Castro, Alejandra and Keller, Christoph A. and M\"uhlmann, Beatrix J.},
    title = "{Siegel Paramodular Forms from Exponential Lifts: Slow versus Fast Growth}",
    eprint = "1910.05353",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "CERN-TH-2019-163",
    month = "10",
    year = "2019"
}
@article{HokPunYu:2009hpy,
    author = "Xiaowei Wang and Hok Pun Yu",
    title = "{Theta function and Bergman metric on Abelian varieties}",
}
@book{Griffiths:433962,
      author        = "Griffiths, Phillip A and Harris, Joseph",
      title         = "{Principles of algebraic geometry}",
      publisher     = "Wiley",
      address       = "New York, NY",
      series        = "Wiley classics library",
      year          = "1994",
      url           = "https://cds.cern.ch/record/433962",
}
@article{Belin:2019jqz,
    author = {Belin, Alexandre and Castro, Alejandra and Keller, Christoph A. and M\"uhlmann, Beatrix J.},
    title = "{Siegel Paramodular Forms from Exponential Lifts: Slow versus Fast Growth}",
    eprint = "1910.05353",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "CERN-TH-2019-163",
    month = "10",
    year = "2019"
}

@article{Belin:2018oza,
    author = "Belin, Alexandre and Castro, Alejandra and Gomes, Joao and Keller, Christoph A.",
    title = "{Siegel paramodular forms and sparseness in AdS$_{3}$/CFT$_{2}$}",
    eprint = "1805.09336",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP11(2018)037",
    journal = "JHEP",
    volume = "11",
    pages = "037",
    year = "2018"
}
@article{Belin:2016knb,
    author = "Belin, Alexandre and Castro, Alejandra and Gomes, Joao and Keller, Christoph A.",
    title = "{Siegel Modular Forms and Black Hole Entropy}",
    eprint = "1611.04588",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP04(2017)057",
    journal = "JHEP",
    volume = "04",
    pages = "057",
    year = "2017"
}
@article{Gopakumar:1998ki,
    author = "Gopakumar, Rajesh and Vafa, Cumrun",
    editor = "Vafa, Cumrun and Yau, S. -T.",
    title = "{On the gauge theory / geometry correspondence}",
    eprint = "hep-th/9811131",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-98-A078",
    doi = "10.4310/ATMP.1999.v3.n5.a5",
    journal = "Adv. Theor. Math. Phys.",
    volume = "3",
    pages = "1415--1443",
    year = "1999"
}
@inproceedings{Kawai:1997em,
    author = "Kawai, Toshiya",
    title = "{K3 surfaces, Igusa cusp form and string theory}",
    booktitle = "{Taniguchi Symposium on Topological Field Theory, Primitive Forms and Related Topics}",
    eprint = "hep-th/9710016",
    archivePrefix = "arXiv",
    reportNumber = "RIMS-1165",
    month = "10",
    year = "1997"
}
@article{Minahan:1998vr,
    author = "Minahan, J. A. and Nemeschansky, D. and Vafa, C. and Warner, N. P.",
    title = "{E strings and N=4 topological Yang-Mills theories}",
    eprint = "hep-th/9802168",
    archivePrefix = "arXiv",
    reportNumber = "USC-98-002, HUTP-A012",
    doi = "10.1016/S0550-3213(98)00426-X",
    journal = "Nucl. Phys. B",
    volume = "527",
    pages = "581--623",
    year = "1998"
}
@article{Eguchi:2011aj,
    author = "Eguchi, Tohru and Hikami, Kazuhiro",
    title = "{Twisted Elliptic Genus for K3 and Borcherds Product}",
    eprint = "1112.5928",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/s11005-012-0569-2",
    journal = "Lett. Math. Phys.",
    volume = "102",
    pages = "203--222",
    year = "2012"
}

@article{Borcherds:1996uda,
    author = "Borcherds, Richard E.",
    title = "{Automorphic forms with singularities on Grassmannians}",
    eprint = "alg-geom/9609022",
    archivePrefix = "arXiv",
    doi = "10.1007/s002220050232",
    journal = "Invent. Math.",
    volume = "132",
    pages = "491--562",
    year = "1998"
}
@article{Borcherds1995,
author = {Borcherds, Richard E.},
journal = {Inventiones mathematicae},
keywords = {automorphic forms; denominator function; generalized Kac-Moody algebra; unimodular lattices; reflection groups; elliptic modular function; Eisenstein series; infinite products; Jacobi forms; Hecke operators; Jacobi groups; Macdonald identities; Weierstrass function},
number = {1},
pages = {161-214},
title = {Automorphic forms on Os + 2,2(R) and infinte products.},
url = {http://eudml.org/doc/144273},
volume = {120},
year = {1995},
}
@article{Moore:1997pc,
    author = "Moore, Gregory W. and Witten, Edward",
    title = "{Integration over the u plane in Donaldson theory}",
    eprint = "hep-th/9709193",
    archivePrefix = "arXiv",
    reportNumber = "IASSNS-HEP-97-97, YCTP-P9-97",
    doi = "10.4310/ATMP.1997.v1.n2.a7",
    journal = "Adv. Theor. Math. Phys.",
    volume = "1",
    pages = "298--387",
    year = "1997"
}
